Refining Fast Calorimeter Simulations with a Schr\"{o}dinger Bridge

Machine learning-based simulations, especially calorimeter simulations, are promising tools for approximating the precision of classical high energy physics simulations with a fraction of the generation time. Nearly all methods proposed so far learn neural networks that map a random variable with a known probability density, like a Gaussian, to realistic-looking events. In many cases, physics events are not close to Gaussian and so these neural networks have to learn a highly complex function. We study an alternative approach: Schr\"{o}dinger bridge Quality Improvement via Refinement of Existing Lightweight Simulations (SQuIRELS). SQuIRELS leverages the power of diffusion-based neural networks and Schr\"{o}dinger bridges to map between samples where the probability density is not known explicitly. We apply SQuIRELS to the task of refining a classical fast simulation to approximate a full classical simulation. On simulated calorimeter events, we find that SQuIRELS is able to reproduce highly non-trivial features of the full simulation with a fraction of the generation time.

==> temp.tex <==


@article{ATLAS:2021pzo,
    author = "Aad, Georges and others",
    collaboration = "ATLAS",
    title = "{AtlFast3: The Next Generation of Fast Simulation in ATLAS}",
    eprint = "2109.02551",
    archivePrefix = "arXiv",
    primaryClass = "hep-ex",
    reportNumber = "CERN-EP-2021-174",
    doi = "10.1007/s41781-021-00079-7",
    journal = "Comput. Softw. Big Sci.",
    volume = "6",
    number = "1",
    pages = "7",
    year = "2022"
}

@article{ATLAS:2021pzo,
    author = "Aad, Georges and others",
    collaboration = "ATLAS",
    title = "{AtlFast3: The Next Generation of Fast Simulation in ATLAS}",
    eprint = "2109.02551",
    archivePrefix = "arXiv",
    primaryClass = "hep-ex",
    reportNumber = "CERN-EP-2021-174",
    doi = "10.1007/s41781-021-00079-7",
    journal = "Comput. Softw. Big Sci.",
    volume = "6",
    number = "1",
    pages = "7",
    year = "2022"
}


@inproceedings{Cresswell:2022tof,
    author = "Cresswell, Jesse C. and Ross, Brendan Leigh and Loaiza-Ganem, Gabriel and Reyes-Gonzalez, Humberto and Letizia, Marco and Caterini, Anthony L.",
    title = "{CaloMan: Fast generation of calorimeter showers with density estimation on learned manifolds}",
    booktitle = "{36th Conference on Neural Information Processing Systems}",
    eprint = "2211.15380",
    archivePrefix = "arXiv",
    primaryClass = "hep-ph",
    month = "11",
    year = "2022"
}


@article{geant4,
title = "Geant4 - a simulation toolkit",
journal = "Nuclear Instruments and Methods in Physics Research Section A: Accelerators, Spectrometers, Detectors and Associated Equipment",
volume = "506",
number = "3",
pages = "250 - 303",
year = "2003",
issn = "0168-9002",
doi = "https://doi.org/10.1016/S0168-9002(03)01368-8",
url = "http://www.sciencedirect.com/science/article/pii/S0168900203013688",
author = "S. Agostinelli and others",
keywords = "Simulation, Particle interactions, Geometrical modelling, Software engineering, Object-oriented technology, Distributed software development"
}

@article{Diefenbacher:2023vsw,
    author = "Diefenbacher, Sascha and Eren, Engin and Gaede, Frank and Kasieczka, Gregor and Krause, Claudius and Shekhzadeh, Imahn and Shih, David",
    title = "{L2LFlows: Generating High-Fidelity 3D Calorimeter Images}",
    eprint = "2302.11594",
    archivePrefix = "arXiv",
    primaryClass = "physics.ins-det",
    month = "2",
    year = "2023"
}

@article{ATLAS:2022jhk,
    collaboration = "ATLAS",
    title = "{Deep generative models for fast photon shower simulation in ATLAS}",
    eprint = "2210.06204",
    archivePrefix = "arXiv",
    primaryClass = "hep-ex",
    reportNumber = "CERN-EP-2022-185",
    month = "10",
    year = "2022"
}

@article{ATLAS:2021pzo,
    author = "Aad, Georges and others",
    collaboration = "ATLAS",
    title = "{AtlFast3: the next generation of fast simulation in ATLAS}",
    eprint = "2109.02551",
    archivePrefix = "arXiv",
    primaryClass = "hep-ex",
    reportNumber = "CERN-EP-2021-174",
    doi = "10.1007/s41781-021-00079-7",
    journal = "Comput. Softw. Big Sci.",
    volume = "6",
    pages = "7",
    year = "2022"
}
